Exploring Efficient Foundational Multi-modal Models for Video Summarization

Foundational models are able to generate text outputs given prompt instructions and text, audio, or image inputs. Recently these models have been combined to perform tasks on video, such as video summarization. Such video foundation models perform pre-training by aligning outputs from each modality-specific model into the same embedding space. Then the embeddings from each model are used within a language model, which is fine-tuned on a desired instruction set. Aligning each modality during pre-training is computationally expensive and prevents rapid testing of different base modality models. During fine-tuning, evaluation is carried out within in-domain videos where it is hard to understand the generalizability and data efficiency of these methods. To alleviate these issues we propose a plug-and-play video language model. It directly uses the texts generated from each input modality into the language model, avoiding pre-training alignment overhead. Instead of fine-tuning we leverage few-shot instruction adaptation strategies. We compare the performance versus the computational costs for our plug-and-play style method and baseline tuning methods. Finally, we explore the generalizability of each method during domain shift and present insights on what data is useful when training data is limited. Through this analysis, we present practical insights on how to leverage multi-modal foundational models for effective results given realistic compute and data limitations.

==> tables/cross_data_perf.tex <==
\begin{table}[t]
    \centering
    \tiny
    \begin{tabular}{c | c c | c c c| c c c | c c c}
    \toprule
    \multicolumn{3}{c}{} & \multicolumn{3}{c}{Cat=Furniture} & \multicolumn{3}{c}{Cat=Electical} & \multicolumn{3}{c}{Cat=Vehicle} \\
    Model & Y $\rightarrow$ C & C $\rightarrow$ Y & Cat & All-Cat & All & Cat & All-Cat & All & Cat & All-Cat & All\\
    \midrule
    Random &  & 15.60 &  &  & 19.74 &  &  &  &  &  &  \\
    Search &  & 20.82 &  &  &  &  &  &  &  &  &  \\
    LoRA \
    \midrule
    ChatBridge \\
    \bottomrule    
    \end{tabular}
    \caption{On the left we compare the performance of using prompts and trained models from YouCook (Y) to test on COIN (C) and vice versa. On the right we ablate the validation performances in subcategories (Cat) of data in COIN. In this setup we search/train on the same category only (Cat), all categories besides the test category (All-Cat), and on all categories (All). Here we report the METEOR scores, and use ALI modalities for \model.}
    \label{tab:cross_data_30b}
\end{table}

==> tables/generation_results.tex <==
\begin{table}[t]
    \centering
    \tiny
    \begin{tabular}{c c | c c c c c | c c c c c}
    \toprule
    \multicolumn{2}{c}{} & \multicolumn{5}{c}{YouCookII} & \multicolumn{5}{c}{COIN} \\
    Model & Modalities & BLEU-1 & BLEU-2 & BLEU-3 & METEOR & ROUGE-L & BLEU-1 & BLEU-2 & BLEU-3 & METEOR & ROUGE-L \\
    \midrule
    \model & R:A & 26.84 & 13.57 & 6.32 & 25.93 & 32.20 & 18.21 & 4.79 & 1.13 & 14.85 & 22.30 \\
    \model & R:AL & 24.22 & 12.09 & 5.73 & 23.69 & 30.53 & 22.96 & 8.83 & 2.33 & 19.97 & 27.85 \\
    \model & R:ALI & 24.45  & 11.89 & 5.11 & 23.55 & 30.38 & 24.77 & 9.89 & 2.73 & 22.024 & 29.75 \\
    \model & R:ALIO & 25.39  & 12.08 & 4.80 & 23.70 & 30.18 & 26.21 & 10.81 & 3.13 & 22.90 & 30.76 \\
    \midrule
    \model & S:A & 33.99  & 18.51 & 9.56 & 34.69 & 36.06 & 17.39 & 4.41 & 1.08 & 14.19 & 20.63 \\
    \model & S:AL & 33.38  & 17.96 & 8.51 & 34.29 & 35.14 & 22.65 & 8.85 & 2.77 & 19.76 & 27.28 \\
    \model & S:ALI & 33.90  & 18.15 & 8.22 & 32.97 & 35.92 & 27.16 & 11.74 & 3.98 & 24.58 & 31.43 \\
    \model & S:ALIO & 29.95  & 15.05 & 6.85 & 30.77 & 32.65 & 25.28 & 10.31 & 2.89 & 23.35 & 29.21 \\
    \midrule
    \model & L:ALI & - \\
    \model & L:ALIO & - \\
    \midrule
    ChatBridge & ALI & - \\
    Vid2Seq & ALI & - \\
    \bottomrule
    \end{tabular}
    \caption{Generation performance on Youcook and COIN datasets. For \model{} we ablate different few shot and training strategies and compare performance against existing works. For few shot inputs, we test randomly selecting sample modalities (R:) versus using a search strategy (S). We also test optimizing the model using LoRA (L:). The modalities we test are the automatic speech recognition outputs (A), the label of the video (L), the image caption (I) as well as objects detected from the scene (O).}
    \label{tab:gen_results}
\end{table}

==> tables/model_change.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c c | c c }
    \toprule
    Substitution & Method & $\Delta$ YouCook & $\Delta$ COIN \\
    \midrule
    \multirow{3}{*}{NewModel (Image)} & \model \\
     & ChatBridge Stg. 2 \\
     & ChatBridge Stg 1+2 \\
     \midrule
     \multirow{3}{*}{NewModel (Audio)} & \model \\
     & ChatBridge Stg. 2 \\
     & ChatBridge Stg 1+2 \\
    \bottomrule
    \end{tabular}
    \caption{We substitute the modality models with different models in each video modeling method. For image models, we use NewModel and for audio we use NewModel. We test the change in performance from the original score.}
    \label{tab:my_label}
\end{table}
